FT K-means: A High-Performance K-means on GPU with Fault Tolerance

K-means is a widely used algorithm in clustering, however, its efficiency is primarily constrained by the computational cost of distance computing. Existing implementations suffer from suboptimal utilization of computational units and lack resilience against soft errors. To address these challenges, we introduce FT K-means, a high-performance GPU-accelerated implementation of K-means with online fault tolerance. We first present a stepwise optimization strategy that achieves competitive performance compared to NVIDIA's cuML library. We further improve FT K-means with a template-based code generation framework that supports different data types and adapts to different input shapes. A novel warp-level tensor-core error correction scheme is proposed to address the failure of existing fault tolerance methods due to memory asynchronization during copy operations. Our experimental evaluations on NVIDIA T4 GPU and A100 GPU demonstrate that FT K-means without fault tolerance outperforms cuML's K-means implementation, showing a performance increase of 10\%-300\% in scenarios involving irregular data shapes. Moreover, the fault tolerance feature of FT K-means introduces only an overhead of 11\%, maintaining robust performance even with tens of errors injected per second.

==> Sections/_outdated_Section3-Algorithm.tex <==
 \begin{figure*}[ht]
     \centering
     \includegraphics[width=\linewidth]{figs/two_side_ABFT.pdf}
     \caption{What is the benefit of two-sided ABFT? Delayed Batched Correction }
     \label{fig:why-two-sided-abft}
     \vspace{0mm}
 \end{figure*}
\section{Two-sided Checksum}
Figure \ref{tab:illustrtation} details our motivation and algorithm designs. Previous FT-FFT, either offline or online, requires \textit{per-signal checksum}, namely applying the encoding vector to each input. Other than that, previous work states that a time-redundant recomputation is necessary. Motivated by the error propagation issue, we find the single error in FFT, although it corrupts hundreds of elements, the errors in the output are proportional to the initial error, as shown in the blue region in Figure \ref{tab:illustrtation}. To avoid frequent checksum encoding, we employ another encoding vector $\mathbf{e}_3=(1,2,\cdots,N)$ to \textit{linear combine} a batch of inputs within each thread and encode those thread-local variables with $\mathbf{e}_1$ at a fixed interval. The corrupted input can be located using a quotient shown in the green region of Figure \ref{tab:illustrtation}.


% \begin{table}[h]
% \centering
% \begin{tabular}{|p{0.11\linewidth}|p{0.25\linewidth}|p{0.06\linewidth}|p{0.30\linewidth}|p{0.11\linewidth}|}
% \hline
% \multirow{2}{*}{ABFT} & \multicolumn{2}{c|}{Error Detection} &\multicolumn{2}{c|}{Error Correction} \\ 
% \cline{2-5}
% & Computation & \#Ops & Computation & \#Ops  \\
% \hline
% \textcolor{blue}{1-sided} &  $(e^TW)X$,$e^T(WX)$ & $8n$ & $WX$ & $5n\log_2n$\\ 
% \hline
% 2-sided &  $(e^TW)X, W(Xe)$ $e^T(WX), (WX)e$ & $16n$ & $\Delta$$= W(Xe) - (WX)e$ $X\leftarrow X+\Delta$& $4n + 5n\log_2n$\\ 
% \hline
% \end{tabular}
% \caption{One-side ABFT vs. Two-sided ABFT}
% \label{table:alg}
% \vspace{0mm}
% \end{table}

% We present our fault model before moving on to the fault tolerance design. This work focuses on the detection of errors in the computing units that can corrupt the results of the output signals. We assume the memory is protected by the ECC code. To robustly tackle these computational inconsistencies at run-time, we have devised a fault-tolerant scheme that operates under the assumption of a single-event upset (SEU). This assumption constrains the model to consider only one soft error in each error detection and correction period. The SEU assumption is not merely a theoretical convenience; it is a well-established and widely employed fault model in numerous research works \cite{reis2005swift, zhai2021ft, ding2011matrix, wu2014ft}. Its validity is corroborated by the empirically observed low occurrence rate of multiple soft errors, a phenomenon attributable to the brief intervals used in fault detection.

\subsection{Error Dectection}

 \begin{equation}
    X\xrightarrow[]{two-sided}X^c:=\begin{bmatrix}X &  X\mathbf{e}\end{bmatrix},
    \label{eqn:two_side_X}
\end{equation}
\begin{equation}
Y^c = W^c\cdot X^c = \begin{bmatrix}WX & WX\mathbf{e} \\ \mathbf{e}^T W\mathbf{x} & \mathbf{e}^TWX\mathbf{e} \end{bmatrix} = \begin{bmatrix}Y & Y\mathbf{e} \\ \mathbf{e}^TY & \mathbf{e}^TY\mathbf{e}
 \end{bmatrix},
\label{eqn:two_side_Y}
\end{equation}
There are two checksums being computed in the two-sided ABFT, namely the left-side $eWX$ and the right-side $WXe$. The checksum along the individual signal, namely one column in $X$, is used to detect the location of the error. Once a mismatch between the checksum before and after one FFT process, it is treated as an error. If an error is detected, then the divergence of the checksum along different signals between before and after the FFT is added back to the detected signal to perform the correction. According to Figure \ref{tab:illustrtation}, both two-sided ABFT and one-sided ABFT compute the checksum on the left side, i.e., eWX. In one-sided ABFT, this checksum is used to detect whether an error has occurred, and if an error is detected, the process reverts to a previously saved state for recalculation. In two-sided ABFT, while using this left-side checksum, the sum is also taken along the row direction of the current data X. If we perform an FFT operation on this checksum vector and subtract it from the checksum of the output result, we can then obtain the correction value for the entire column of erroneous data. Next, we just need to add this correction value back to correct the error.



 \subsection{Delayed Batched Correction}
The biggest difference between one-sided ABFT and two-sided ABFT is whether there is an immediate need for recalculation. From Fig. \ref{tab:illustrtation}, we understand that two-sided ABFT requires the calculation of an additional set of checksums, and correction also involves performing an FFT operation on the checksum vector. So, compared to one-sided ABFT, where does the advantage of two-sided ABFT lie? This work points to the advantage, namely delayed batched correction.

Under the assumptions of ABFT, a single checksum can correct one error. Therefore, for two-sided ABFT, it is only necessary to note the position of the error, i, and then continue processing the data for position i+1, until the operation ends or a new error occurs. In those cases, we need to correct the contents of the checksum at the erroneous position $i$. As a result, there is an opportunity for batch-processing operations among different threads, which enhances parallelism. Moreover, since there is no need to stop and execute immediately, the running pipeline of the program is not affected, thereby avoiding stalls.
 Figure \ref{fig:why-two-sided-abft} illustrates the difference between one-sided ABFT and two-sided ABFT. Any fault tolerance mechanism is essentially a tradeoff between resources. Compared to one-sided ABFT, two-sided ABFT actually uses additional computation to reduce memory overhead. If one-sided ABFT chooses not to recalculate immediately, it will need to reload data from the storage device during the next computation. In contrast, two-sided ABFT \textit{compresses} the data already read into local registers in the form of checksums. Therefore, before a new error occurs, the error information can be decompressed at any time by the checksum and used to correct previous errors. 

Fig. \ref{tab:illustrtation} demonstrates the capability of batch delay correction. The 2$\times$2 grid in the figure represents a warp. When thread 1 in a warp encounters an error, the entire warp can continue to operate normally until the program terminates or a new error occurs. In contrast, one-sided ABFT requires immediate re-execution, otherwise it would need to reload data from memory.

 Figure \ref{tab:illustrtation} details the computation process for two-sided ABFT. When an error occurs, a thread can note that an error has occurred at this point. Error correction operations are only carried out when the next error occurs or when the program terminates. Placing the right-side checksum at the end of the loop is to prevent a potential second error from contaminating the checksum that has already recorded one error.
% \begin{algorithm}
% \caption{Two-Sided ABFT FFT Algorithm}
% \begin{algorithmic}[1]
% \Procedure{Two-Sided-ABFT-FFT}{}
% \State Get initial radix $k$ and corresponding $m = \frac{N}{k}$
% \State Calculate left checksum vector $c_m = e_m W_m$
% \State Set the error flag $ErrFlag = \text{false}$
%     \State Set the error location $j = \text{-1}$
% \For{$i \text{ from } 0 \text{ to } k-1$}
%         \State Calculate the $i$-th FFT: $X'_i = W_m x_i$
%         \If {$(\lVert e_m X'_i - c_m x_i \rVert > \eta_1)$ or $i == k-1$}
%         \If {$ErrFlag$}
%         \State Correction $X'_j -= W_m r_m - p_m$
%         \EndIf
%         \State Set error flag $Errflag=True$
%         \State Record error location $j = i$
%         \EndIf
%         \State Calculate right checksum vector $p_m += X'_ie_m$
%          \State Calculate right checksum vector $r_m +=  x_i e_m$
% \EndFor
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}



==> listing/alg-interp.tex <==
\begin{lstlisting}[language=python, caption={The essense of {\ginterp} implementation.}, basicstyle=\ttfamily\footnotesize, 
escapeinside={(*@}{@*)}, morekeywords={fn, reference, volatile, constexpr, parfor},
label={cuszinterp::algo::interp}
]
""" original data value (*@$d$@*), predicted value (*@$p$@*), 
predict. error (*@$e$@*), quant-code (*@$q$@*), error bound (*@$eb$@*), 
radius (*@$r$@*). We refer reader to Tao et al. 
2017 for the detailed pred-quant. algorithm."""
 
fn PerPointPredQuant<sym Direction>(volatile (*@$shm\{data, quant\}$@*), (*@$x$@*), (*@$y$@*), (*@$z$@*), (*@$\alpha$@*)):
    reference (*@$(d, q) \gets (shm.data_{z,y,x}, shm.quant_{z,y,x})$@*)
    (*@$p \gets$@*) Interp<Direction>((*@$x$@*), (*@$y$@*), (*@$z$@*), (*@$\alpha$@*))
    if constexpr COMPRESS: 
        QuantizeComppress((*@$d$@*), (*@$p$@*), (*@$q$@*))
    if constexpr DECOMPRESS: 
        QuantizeDecompress((*@$d$@*), (*@$p$@*), (*@$q$@*))

fn Stage<class Map>(..., Map map):
    if constexpr CORSENING:
        multiply call PerPointPredQuant(...) 
    else:
        one-time call PerPointPredQuant(...)

fn InterpolateIter(volatile (*@$shm\{data, quant\}$@*):
    parfor (*@$\alpha \gets \{4,2,1\}$@*) (predefined parallelism):
        for constexpr (*@$i \gets \{0,1,2\}$@*):
            Stage<(*@$i$@*)>(...)
\end{lstlisting}

==> listing/alg-pred-quant.tex <==
\begin{algorithmic}[1]

	\Statex \textbf{notation:} original data element/value $d$, predicted value $p$, prediction error $e$, quant-code $q$, error bound $eb$,  radius $r$ %(global or captured)

	\Statex
	\Procedure{CompressPredQuant}{\REFERENCE{} $d$, $p$, \REFERENCE{} $q$}
	\State $e \gets d-p$
	\State code $\gets$ \textsc{fabs}($e$)$\,\div\,eb + 1$; code $\gets$ $-$code \INLINEIF{} $e<0$
	\State code $\gets$ \textsc{int}(code$\,\div\,2$) $+\,r$
	\State $q \gets$ code; $d \gets p + (\text{code} - r) \times eb\cdot2$
	\EndProcedure

	\Statex

	\Procedure{DecompressPredQuant}{\REFERENCE{} $d$, $p$, \REFERENCE{} $q$}
	\State $d \gets p + (q - r) \times eb\cdot2$
	\EndProcedure

	\Statex

\end{algorithmic}

==> listing/cr-same-eb-NO-bitcomp.tex <==
\newcommand{\TabDataName}[1]{\rotatebox{90}{\bfseries\scriptsize\scalebox{0.8}{#1}}}
\setlength{\tabcolsep}{4pt}
\scriptsize
\begin{tabular}{|l@{}c|r|r|r|r|r|r|}
  % \hline
  % \multirow{2}{*}{\textbf{Dataset}} &
  % \multirow{2}{*}{\textbf{epsilon}} &
  % \multirow{2}{*}{\textbf{cuSZ}}    &
  % \multirow{2}{*}{\textbf{cuSZp}}   &
  % \multirow{2}{*}{\textbf{cuSZx}}   &
  % \multirow{2}{*}{\textbf{FZ-GPU}}  &
  % \multirow{2}{*}{\textbf{cuSZ-I}}  &
  % \textbf{Improve}                                                                                                                                     \\
  %                                   &       &                     &                     &               &               &                     &
  % \textbf{(\%)}                                                                                                                                        \\

  \multicolumn{1}{l}{\rotatebox{90}{\textbf{Dataset}}} &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{epsilon}}} &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZ}}}    &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZp}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZx}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{FZ-GPU}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZ-I}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{Improve \%}}}
  \\
  % \hline
  \hline
  \multirow{3}{*}{\TabDataName{RTM}}                   & 1E--2 & 28.7                & \SecondbestCr{41.6} & \NoBcBestCr{53.7} & 32.0              & 28.8                & --46.4 \\ \cline{3-8}
                                                       & 1E--3 & 24.7                & 19.8                & \NoBcBestCr{30.7} & 20.9              & \SecondbestCr{27.4} & --10.7 \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{17.7} & 10.7                & 17.4              & 12.1              & \NoBcBestCr{21.5}   & 21.5   \\ \hline
  \multirow{3}{*}{\TabDataName{Miranda}}               & 1E--2 & 27.1                & 16.8                & 7.9               & \NoBcBestCr{30.6} & \SecondbestCr{28.5} & --6.9  \\ \cline{3-8}
                                                       & 1E--3 & \SecondbestCr{22.9} & 9.6                 & 5.1               & 19.2              & \NoBcBestCr{26.3}   & 14.8   \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{15.3} & 6.0                 & 3.6               & 11.8              & \NoBcBestCr{19.5}   & 27.5   \\ \hline
  \multirow{3}{*}{\TabDataName{S3D}}                   & 1E--2 & \SecondbestCr{28.0} & 7.2                 & 19.5              & 15.5              & \NoBcBestCr{29.5}   & 5.4    \\ \cline{3-8}
                                                       & 1E--3 & \SecondbestCr{23.3} & 4.5                 & 9.3               & 11.8              & \NoBcBestCr{28.8}   & 23.6   \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{17.3} & 3.1                 & 5.0               & 9.0               & \NoBcBestCr{26.0}   & 50.3   \\ \hline
  \multirow{3}{*}{\TabDataName{NYX}}                   & 1E--2 & \NoBcBestCr{30.2}   & 20.3                & N/A               & 25.3              & \SecondbestCr{29.6} & --2.0  \\ \cline{3-8}
                                                       & 1E--3 & \SecondbestCr{23.9} & 9.6                 & N/A               & 14.4              & \NoBcBestCr{28.0}   & 17.2   \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{15.3} & 5.7                 & N/A               & 8.4               & \NoBcBestCr{18.7}   & 22.2   \\ \hline
  \multirow{3}{*}{\TabDataName{JHTDB}}                 & 1E--2 & \SecondbestCr{26.6} & 10.3                & 3.0               & 12.1              & \NoBcBestCr{29.3}   & 10.2   \\ \cline{3-8}
                                                       & 1E--3 & \SecondbestCr{17.7} & 5.4                 & 2.5               & 9.9               & \NoBcBestCr{25.2}   & 42.4   \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{10.7} & 3.5                 & 1.8               & 6.4               & \NoBcBestCr{13.3}   & 24.3   \\ \hline
  \multirow{3}{*}{\TabDataName{Qmcpack}}               & 1E--2 & \SecondbestCr{28.6} & 22.2                & 3.3               & 19.0              & \NoBcBestCr{29.3}   & 2.4    \\ \cline{3-8}
                                                       & 1E--3 & \SecondbestCr{20.9} & 10.1                & 2.5               & 12.1              & \NoBcBestCr{27.7}   & 32.5   \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{14.8} & 5.6                 & 1.9               & 8.3               & \NoBcBestCr{22.6}   & 52.7   \\ \hline
\end{tabular}

==> listing/cr-same-eb-bitcomp.tex <==

\begin{tabular}{|l|c|r|r|r|r|r|r|}
  \hline
  \multirow{2}{*}{\textbf{Dataset}} &
  \multirow{2}{*}{\textbf{epsilon}} &
  \multirow{2}{*}{\textbf{cuSZ}}    &
  \multirow{2}{*}{\textbf{cuSZp}}   &
  \multirow{2}{*}{\textbf{cuSZx}}   &
  \multirow{2}{*}{\textbf{FZ-GPU}}  &
  \multirow{2}{*}{\textbf{cuSZ-I}}  &
  \textbf{Improve}                                                                                                              \\
                                    &       &                     &                      &      &      &                &
  \textbf{(\%)}                                                                                                                 \\
  \hline
  \hline
  \multirow{3}{*}{\textbf{RTM}}     & 1E--2 & 84.1                & \SecondbestCr{100.5} & 70.4 & 69.7 & \BestCr{234.0} & 132.8 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{50.2} & 31.1                 & 38.8 & 35.5 & \BestCr{96.2}  & 91.6  \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{26.6} & 14.0                 & 21.4 & 18.4 & \BestCr{45.4}  & 70.7  \\ \hline
  \multirow{3}{*}{\textbf{MIRANDA}} & 1E--2 & \SecondbestCr{67.4} & 18.7                 & 8.1  & 43.9 & \BestCr{174.0} & 158.2 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{38.5} & 10.7                 & 5.2  & 27.1 & \BestCr{77.2}  & 100.5 \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{19.8} & 6.7                  & 3.7  & 15.4 & \BestCr{34.3}  & 73.2  \\ \hline
  \multirow{3}{*}{\textbf{S3D}}     & 1E--2 & \SecondbestCr{42.5} & 18.9                 & 19.9 & 25.6 & \BestCr{245.0} & 476.5 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{28.3} & 8.8                  & 9.5  & 16.1 & \BestCr{137.0} & 384.1 \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{19.0} & 5.0                  & 5.1  & 11.6 & \BestCr{58.2}  & 206.3 \\ \hline
  \multirow{3}{*}{\textbf{NYX}}     & 1E--2 & 71.6                & \SecondbestCr{95.9}  & N/A  & 84.5 & \BestCr{256.0} & 166.9 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{34.4} & 19.0                 & N/A  & 26.2 & \BestCr{66.1}  & 92.2  \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{17.9} & 7.5                  & N/A  & 12.3 & \BestCr{25.1}  & 40.2  \\ \hline
  \multirow{3}{*}{\textbf{JHTDB}}   & 1E--2 & \SecondbestCr{27.8} & 19.9                 & 3.1  & 18.0 & \BestCr{132.0} & 374.8 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{17.7} & 6.0                  & 2.5  & 11.5 & \BestCr{34.8}  & 96.6  \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{10.7} & 3.6                  & 1.8  & 7.8  & \BestCr{13.3}  & 24.3  \\ \hline
  \multirow{3}{*}{\textbf{QMCPACK}} & 1E--2 & \SecondbestCr{46.0} & 38.7                 & 3.3  & 30.3 & \BestCr{168.0} & 265.2 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{23.7} & 11.5                 & 2.5  & 14.7 & \BestCr{78.7}  & 232.1 \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{15.3} & 5.8                  & 1.9  & 10.2 & \BestCr{34.6}  & 126.1 \\ \hline
\end{tabular}

==> listing/cr-same-eb-combined.tex <==
\begin{tabular}{ >{\color{black}}l@{} >{\color{black}}c| *{2}{c |rrrrr| >{\color{black}}r|} }
  \multicolumn{1}{l}{\rotatebox{90}{\textbf{Dataset}}} &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{epsilon}}} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{\cusz}}}    &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZp}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZx}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{FZ-GPU}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\color{black}\textbf{\thiswork}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\color{black}\textbf{Improve \%}}} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{\cusz}}}    &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZp}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZx}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{FZ-GPU}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\color{black}\textbf{\thiswork}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\color{black}\textbf{Improve \%}}}
  \\
  \cline{1-2}\cline{4-9}\cline{11-16}
  \multirow{3}{*}{\TabDataName{JHTDB}}                 & 1e--2 && \SecondbestCr{26.6} & 10.3                & 3.0               & 12.1              & \NoBcBestCr{29.3}   & 10.2   &  & \SecondbestCr{27.8} & 19.9                 & 3.1  & 18.0 & \BestCr{132.0} & 374.8 \\
                                                       & 1e--3 && \SecondbestCr{17.7} & 5.4                 & 2.5               & 9.9               & \NoBcBestCr{25.2}   & 42.4   &  & \SecondbestCr{17.7} & 6.0                  & 2.5  & 11.5 & \BestCr{34.8}  & 96.6  \\
                                                       & 1e--4 && \SecondbestCr{10.7} & 3.5                 & 1.8               & 6.4               & \NoBcBestCr{13.3}   & 24.3   &  & \SecondbestCr{10.7} & 3.6                  & 1.8  & 7.8  & \BestCr{13.3}  & 24.3  \\

                                                       
   \cline{1-2}\cline{4-9}\cline{11-16}
  \multirow{3}{*}{\TabDataName{Miranda}}               & 1e--2 && 27.1                & 16.8                & 7.9               & \NoBcBestCr{30.6} & \SecondbestCr{28.5} & --6.9  &  & \SecondbestCr{67.4} & 18.7                 & 8.1  & 43.9 & \BestCr{174.0} & 158.2 \\
                                                       & 1e--3 && \SecondbestCr{22.9} & 9.6                 & 5.1               & 19.2              & \NoBcBestCr{26.3}   & 14.8   &  & \SecondbestCr{38.5} & 10.7                 & 5.2  & 27.1 & \BestCr{77.2}  & 100.5 \\
                                                       & 1e--4 && \SecondbestCr{15.3} & 6.0                 & 3.6               & 11.8              & \NoBcBestCr{19.5}   & 27.5   &  & \SecondbestCr{19.8} & 6.7                  & 3.7  & 15.4 & \BestCr{34.3}  & 73.2  \\
  \cline{1-2}\cline{4-9}\cline{11-16}
  \multirow{3}{*}{\TabDataName{NYX}}                   & 1e--2 && \NoBcBestCr{30.2}   & 20.3                & N/A               & 25.3              & \SecondbestCr{29.6} & --2.0  &  & 71.6                & \SecondbestCr{95.9}  & N/A  & 84.5 & \BestCr{256.0} & 166.9 \\
                                                       & 1e--3 && \SecondbestCr{23.9} & 9.6                 & N/A               & 14.4              & \NoBcBestCr{28.0}   & 17.2   &  & \SecondbestCr{34.4} & 19.0                 & N/A  & 26.2 & \BestCr{66.1}  & 92.2  \\
                                                       & 1e--4 && \SecondbestCr{15.3} & 5.7                 & N/A               & 8.4               & \NoBcBestCr{18.7}   & 22.2   &  & \SecondbestCr{17.9} & 7.5                  & N/A  & 12.3 & \BestCr{25.1}  & 40.2  \\
 
  \cline{1-2}\cline{4-9}\cline{11-16}
  \multirow{3}{*}{\TabDataName{Qmcpack}}               & 1e--2 && \SecondbestCr{28.6} & 22.2                & 3.3               & 19.0              & \NoBcBestCr{29.3}   & 2.4    &  & \SecondbestCr{46.0} & 38.7                 & 3.3  & 30.3 & \BestCr{168.0} & 265.2 \\
                                                       & 1e--3 && \SecondbestCr{20.9} & 10.1                & 2.5               & 12.1              & \NoBcBestCr{27.7}   & 32.5   &  & \SecondbestCr{23.7} & 11.5                 & 2.5  & 14.7 & \BestCr{78.7}  & 232.1 \\
                                                       & 1e--4 && \SecondbestCr{14.8} & 5.6                 & 1.9               & 8.3               & \NoBcBestCr{22.6}   & 52.7   &  & \SecondbestCr{15.3} & 5.8                  & 1.9  & 10.2 & \BestCr{34.6}  & 126.1 \\
\cline{1-2}\cline{4-9}\cline{11-16}
  \multirow{3}{*}{\TabDataName{RTM}}                   & 1e--2 && 28.7                & \SecondbestCr{41.6} & \NoBcBestCr{53.7} & 32.0              & 28.8                & --46.4 &  & 84.1                & \SecondbestCr{100.5} & 70.4 & 69.7 & \BestCr{234.0} & 132.8 \\
                                                       & 1e--3 && 24.7                & 19.8                & \NoBcBestCr{30.7} & 20.9              & \SecondbestCr{27.4} & --10.7 &  & \SecondbestCr{50.2} & 31.1                 & 38.8 & 35.5 & \BestCr{96.2}  & 91.6  \\
                                                       & 1e--4 && \SecondbestCr{17.7} & 10.7                & 17.4              & 12.1              & \NoBcBestCr{21.5}   & 21.5   &  & \SecondbestCr{26.6} & 14.0                 & 21.4 & 18.4 & \BestCr{45.4}  & 70.7  \\
  \cline{1-2}\cline{4-9}\cline{11-16}
  
  \multirow{3}{*}{\TabDataName{S3D}}                   & 1e--2 && \SecondbestCr{28.0} & 7.2                 & 19.5              & 15.5              & \NoBcBestCr{29.5}   & 5.4    &  & \SecondbestCr{42.5} & 18.9                 & 19.9 & 25.6 & \BestCr{245.0} & 476.5 \\
                                                       & 1e--3 && \SecondbestCr{23.3} & 4.5                 & 9.3               & 11.8              & \NoBcBestCr{28.8}   & 23.6   &  & \SecondbestCr{28.3} & 8.8                  & 9.5  & 16.1 & \BestCr{137.0} & 384.1 \\
                                                       & 1e--4 && \SecondbestCr{17.3} & 3.1                 & 5.0               & 9.0               & \NoBcBestCr{26.0}   & 50.3   &  & \SecondbestCr{19.0} & 5.0                  & 5.1  & 11.6 & \BestCr{58.2}  & 206.3 \\
  
  \cline{1-2}\cline{4-9}\cline{11-16}
  
\multicolumn{3}{c|}{} & \multicolumn{6}{c|}{\color{black}\bfseries without Bitcomp} & \multicolumn{1}{c|}{} & \multicolumn{6}{c|}{\color{black}\bfseries {with Bitcomp} } \\
\multicolumn{2}{c}{col. no.} & \multicolumn{1}{c}{} &
1 & 2 & 3 & 4       & \multicolumn{1}{r}{5} & \multicolumn{1}{r}{6} & 
\multicolumn{1}{c}{} & 
i & ii & iii & iv   & \multicolumn{1}{r}{v} & \multicolumn{1}{r}{vi} \\
\end{tabular}

==> listing/cuszi-overview.tex <==
\newcommand{\TableNop}{\multicolumn{1}{c}{}}
\begin{tabular}{ l c |p{11em}| c cc|p{5em}|c|p{9.19em}|}
	\TableNop
	                                              & \TableNop
	                                              &
	\multicolumn{1}{p{11em}}{prediction \& error quantization (with outlier compaction)}
	                                              & \TableNop                          &
	\multicolumn{1}{c}{statistics}                & \TableNop
	                                              &
	\multicolumn{3}{c}{multi-stage lossless encoding}                                                                                                                                                          \\
	\cline{3-3}\cline{5-5}\cline{7-9}
	\TableNop                                     & \TableNop                          & \TableNop                      & \TableNop     &                  & \TableNop     & \TableNop & \TableNop & \TableNop \\
	\cline{3-3}\cline{5-5}\cline{7-7}
	\textbf{cusz}                                 &                                    &
	Lorenzo prediction, dual-quantization variant 
	& \multicolumn{1}{c|}{$\rightarrow$} & \multicolumn{1}{c|}{histogram} & $\rightarrow$ & Huffman encoding & \TableNop     & \TableNop                         \\
	\cline{3-3}\cline{5-5}\cline{7-7}
	\TableNop                                     & \TableNop                          & \TableNop                      & \TableNop     &                  & \TableNop     & \TableNop & \TableNop & \TableNop \\
	\cline{3-3}\cline{5-5}\cline{7-7}\cline{9-9}
	\textbf{cusz-i}                               &                                    &
	linear, qudratic, and cubic spline-interpolation
	                                              & \multicolumn{1}{c|}{$\rightarrow$}                 & \multicolumn{1}{c|}{histogram} & $\rightarrow$ & Huffman encoding & $\rightarrow$ &
	spatial-redundancy elimination                                                                                                                                                                             \\
	\cline{3-3}\cline{5-5}\cline{7-7}\cline{9-9}
\end{tabular}%

==> listing/datasets.tex <==
\begin{tabular}{|rrll|}
\hline  \multicolumn{4}{|l|}{\textbf{JHTDB}~\cite{jhtdb}: numerical simulation of turbulence.} \\
% \hline  
& 10 files    & dim: $zyx = 512\times512\times512$          & total: 5 GB    \\
% \hline
\hline  \multicolumn{4}{|l|}{\textbf{Miranda}~\cite{miranda}: hydrodynamics simulation.} \\
% \hline  
& 7 files & dim: $zyx=256\times384\times384$          & total: 1 GB   \\
% \hline
\hline  
\multicolumn{4}{|l|}{\textbf{NYX}~\cite{nyx}: cosmological hydrodynamics simulation.}  \\
% \hline  
& 6 files & dim: $zyx=512\times512\times512$          & total: 3.1 GB \\
% \hline
\hline  
\multicolumn{4}{|l|}{\textbf{QMCPack}~\cite{qmcpack}: Monte Carlo quantum simlation.}  \\
% \hline  
& 1 files & dim: $zyx=288\times115\times69\times69$ & total: 612 MB \\
% \hline
\hline  
\multicolumn{4}{|l|}{\textbf{RTM}~\cite{rtm}: reverse time migration for seismic imaging.} \\
& 37 files     & dim: $zyx=449\times449\times235$          & total: 6.5 GB \\
% \hline
\hline \multicolumn{4}{|l|}{\textbf{S3D}~\cite{repo-sdrbench}: combustion process simulation.}  \\
% \hline 
& 11 files   & dim: $zyx=500\times500\times500$          & total: 5.1 GB \\
\hline
\end{tabular}

==> listing/tab-testbed.tex <==
\begin{tabular}{ | >{\bfseries}l|c|c|c|}
    \hline
    {GPU}      & \multicolumn{2}{c|}{A100 (40GB)}       & A40 (48 GB)        \\
    \hline
    \hline
    {testbed}  & Theta-GPU    & Anvil        & JLSE         \\
    \hline
    {mem. bw.}  & \multicolumn{2}{c|}{1555 GB/s}    & 695.8  GB/s  \\
    \hline
    {compute}  & \multicolumn{2}{c|}{19.49 TFLOPS} & 37.42 TFLOPS \\
    \hline
    {CUDA/driver}     & 11.4/470.161.03         & 11.6/530.30.02         & 11.8/545.23.06         \\
    \hline
    % {driver}   & 470.161.03   & 530.30.02    & 545.23.06    \\
    % \hline
    % {access}   &
    % \multicolumn{3}{c|}{November, 2023}                     \\
    % \hline
\end{tabular}%

